Context Dependent Semantic Parsing: A Survey

Semantic parsing is the task of translating natural language utterances into machine-readable meaning representations. Currently, most semantic parsing methods are not able to utilize contextual information (e.g. dialogue and comments history), which has a great potential to boost semantic parsing performance. To address this issue, context dependent semantic parsing has recently drawn a lot of attention. In this survey, we investigate progress on the methods for the context dependent semantic parsing, together with the current datasets and tasks. We then point out open problems and challenges for future research in this area. The collected resources for this topic are available at:https://github.com/zhuang-li/Contextual-Semantic-Parsing-Paper-List.

==> tab-example-dialog.tex <==
\begin{table}[ht] % title of Table
\centering % used for centering table
{\small
\scalebox{1}{\begin{tabular}{l l} % centered columns (4 columns)
\hline\hline %inserts double horizontal lines
$\text{D}$ & Database about cars \\ % inserts table
%heading
\hline % inserts single horizontal line
$\text{Q}_1$ & What is id of the car with the max horsepower? \\
$\text{S}_1$ & 
SELECT Id FROM CARS\_DATA ORDER BY Horsepower DESC LIMIT 1\\
$\text{Q}_2$ & How about with the max mpg? \\
$\text{S}_2$ & SELECT Id FROM CARS\_DATA ORDER BY MPG DESC LIMIT 1\\
$\text{Q}_3$ & Show its Make! \\
$\text{S}_3$ & SELECT T1.Make FROM CAR\_NAMES AS T1 JOIN CARS\_DATA \\& 
AS T2 ON T1.MakeId = T2.Id ORDER BY T2.MPG DESC LIMIT 1\\
\hline %inserts single line
\end{tabular}
}}
\caption{An interaction annotated with SQL queries from \Sparc. Given an external database $D$, the user question $Q_i$ would be parsed into a SQL query $S_i$.}
\label{tab:CoSQL} % is used to refer this table in the text
 \vspace{-4mm}
\end{table}

==> tab-example-dialog_1.tex <==
\begin{table}[ht] % title of Table
\centering % used for centering table
{\small
\scalebox{1}{\begin{tabular}{l l} % centered columns (4 columns)
\hline\hline %inserts double horizontal lines
$\text{D}$ & Database about air travel information \\ % inserts table
%heading
\hline % inserts single horizontal line
$\text{Q}_1$ & show me flights from seattle to boston next monday? \\
$\text{S}_1$ & 
%(SELECT DISTINCT flight.flight\_id FROM flight WHERE (flight.from\_airport IN (SELECT airport\_service.airport\_code \\& FROM airport\_service WHERE airport\_service.city\_code IN (SELECT city.city\_code FROM city WHERE city.city\_name \\& 
%= ’SEATTLE’))) AND (flight.to\_airport IN (SELECT airport\_service.airport\_code FROM airport\_service WHERE \\& airport\_service.city\_code IN (SELECT city.city\_code FROM city WHERE city.city\_name = ’BOSTON’))) AND \\& (flight.flight\_days IN (SELECT days.days\_code FROM days WHERE days.day name IN (SELECT date\_day.day\_name \\&
%FROM date\_day WHERE date\_day.year = 1993 AND date\_day.month\_number = 2 AND date\_day.day\_number = 8)))); \\
(SQL expressions)\\
$\text{A}_1$ & (Result table with 31 flights) \\
$\text{Q}_2$ & on american airlines. \\
$\text{S}_2$ & 
%(SELECT DISTINCT flight.flight\_id FROM flight WHERE (flight.airline\_code = ’AA’) AND (flight.from\_airport \\& 
%IN (SELECT airport\_service.airport code FROM airport\_service WHERE airport\_service.city\_code IN (SELECT \\& city.city\_code FROM city WHERE city.city\_name = ’SEATTLE’))) AND (flight.to\_airport IN (SELECT \\& airport\_service.airport\_code FROM airport\_service WHERE airport\_service.city\_code IN (SELECT \\&
%city.city\_code FROM city WHERE city.city\_name = ’BOSTON’))) AND (flight.flight\_days IN (SELECT \\&
%days.days\_code FROM days WHERE days.day\_name IN (SELECT date\_day.day name FROM date\_day WHERE \\&
%date\_day.year = 1993 AND date\_day.month\_number = 2 AND date\_day.day\_number = 8)))); \\
(SQL expressions)\\
$\text{A}_2$ & (Result table with 5 flights) \\
$\text{Q}_3$ & which ones arrive at 7pm? \\
$\text{S}_3$ & 
%(SELECT DISTINCT flight.flight\_id FROM flight WHERE (flight.airline\_code = ’AA’) AND (flight.from\_airport \\&
%IN (SELECT airport\_service.airport\_code FROM airport\_service WHERE airport\_service.city\_code IN (SELECT \\& city.city\_code FROM city WHERE city.city\_name = ’SEATTLE’))) AND (flight.to airport IN (SELECT \\&
%airport\_service.airport\_code FROM airport\_service WHERE airport\_service.city\_code IN (SELECT \\&
%city.city\_code FROM city WHERE city.city\_name = ’BOSTON’))) AND (flight.flight\_days IN (SELECT \\&
%days.days\_code FROM days WHERE days.day\_name IN (SELECT date\_day.day name FROM date\_day WHERE \\&
%date\_day.year = 1993 AND date\_day.month\_number = 2 AND date\_day.day\_number = 8))) AND \\&
%(flight.arrival\_time = 1900)); \\
(SQL expressions)\\
$\text{R}_3$ & (No flights returned) \\
$\text{Q}_4$ & show me delta flights. \\
$\text{S}_4$ & 
%(SELECT DISTINCT flight.flight\_id FROM flight WHERE (flight.airline\_code = ’DL’) AND \\& (flight.from\_airport IN (SELECT airport\_service.airport\_code FROM airport\_service WHERE \\& airport\_service.city\_code IN (SELECT city.city\_code FROM city WHERE city.city\_name = ’SEATTLE’))) AND \\& (flight.to\_airport IN (SELECT airport\_service.airport\_code FROM airport\_service WHERE \\&
%airport\_service.city\_code IN (SELECT city.city\_code FROM city WHERE city.city\_name = ’BOSTON’))) AND \\& (flight.flight days IN (SELECT days.days\_code FROM days WHERE days.day\_name IN (SELECT date\_day.day\_name \\&
%FROM date\_day WHERE date\_day.year = 1993 AND date\_day.month\_number = 2 AND date\_day.day\_number = 8)))); \\
(SQL expressions)\\
$\text{A}_4$ & (Result table with 5 flights) \\
\hline %inserts single line
\end{tabular}
}}
\caption{An interaction annotated with SQL queries from \Atis. Given an external database $D$, the user question $Q_i$ would be parsed into a SQL query $S_i$, returning an answer $A_i$.}
\label{tab:CoSQL} % is used to refer this table in the text
 \vspace{-4mm}
\end{table}

==> tab-example-dialog_backup.tex <==
\begin{table}[ht] % title of Table
\centering % used for centering table
{\small
\scalebox{0.7}{\begin{tabular}{l l l} % centered columns (4 columns)
\hline\hline %inserts double horizontal lines
$\text{D}_1$ & Database about student dormitories containing 5 tables &  \\ % inserts table
%heading
\hline % inserts single horizontal line
$\text{Q}_1$ & What are the names of all the dorms? & INFORM\_SQL \\
\rowcolor{Gray}
$\text{S}_1$ & SELECT dorm\_name FROM dorm &  \\
\rowcolor{Gray}
$\text{A}_1$ & (Result table with many entries) &  \\
\rowcolor{Gray}
$\text{R}_1$ & This is the list of the names of all the dorms. & CONFIRM\_SQL \\
$\text{Q}_2$ & Which of those dorms have a TV lounge? & INFORM\_SQL \\
\cellcolor{Gray}
$\text{S}_2$  & \cellcolor{Gray}  SELECT T1.dorm\_name FROM dorm AS T1 JOIN &\cellcolor{Gray} \\\cellcolor{Gray}  & 
\rowcolor{Gray}
has\_amenity AS T2 ON T1.dormid = T2.dormid JOIN &\\ \cellcolor{Gray} &
\rowcolor{Gray}
dorm\_amenity AS T3 ON T2.amenid = T3.amenid &\\\cellcolor{Gray}  &
\rowcolor{Gray}
WHERE T3.amenity\_name = ‘TV Lounge’ &  \\
\rowcolor{Gray}
$\text{A}_2$ & (Result table with many entries) &  \\
\rowcolor{Gray}
$\text{R}_2$ & This shows the names of dorms with TV lounges. & CONFIRM\_SQL \\
$\text{Q}_3$ & What dorms have no study rooms as amenities? & AMBIGUOUS \\
\rowcolor{Gray}
$\text{R}_3$ & Do you mean among those with TV Lounges? & CLARIFY \\
$\text{Q}_4$ & Yes. & AFFIRM \\
\rowcolor{Gray}
$\text{S}_4$  & SELECT T1.dorm\_name FROM dorm AS T1 JOIN &\\ \cellcolor{Gray} &
\rowcolor{Gray}
has\_amenity AS T2 ON T1.dormid = T2.dormid JOIN &\\ \cellcolor{Gray} &
\rowcolor{Gray}
dorm\_amenity AS T3 ON T2.amenid = T3.amenid &\\ \cellcolor{Gray} &
\rowcolor{Gray}
WHERE T3.amenity\_name = ‘TV Lounge’&\\ \cellcolor{Gray} &
\rowcolor{Gray}
EXCEPT SELECT T1.dorm\_name FROM dorm &\\ \cellcolor{Gray} &
\rowcolor{Gray}
AS T1 JOIN has\_amenity AS T2 ON T1.dormid = T2.dormid &\\ \cellcolor{Gray} &
\rowcolor{Gray}
JOIN dorm\_amenity AS T3 ON T2.amenid = T3.amenid &\\ \cellcolor{Gray} &
\rowcolor{Gray}
WHERE T3.amenity\_name = ‘Study Room’ &  \\
\rowcolor{Gray}
$\text{A}_4$ & Fawlty Towers &  \\
\rowcolor{Gray}
$\text{R}_4$ & Fawlty Towers is the name of the dorm &\\ \cellcolor{Gray} &
\rowcolor{Gray}
that has a TV lounge but not a study &\\ \cellcolor{Gray} &
\rowcolor{Gray}
room as an amenity. & CONFIRM\_SQL \\
&...&\\
$\text{Q}_8$ & Thanks. & THANK\_YOU \\
\rowcolor{Gray}
$\text{R}_8$ & You are welcome. & WELCOME \\
\hline %inserts single line
\end{tabular}
}}
\caption{A dialog annotated with SQL queries and action states in the \Cosql\cite{yu2019cosql}. Given an external database $D_i$, the user question $Q_i$ would be parsed into a SQL query $S_i$, returning an answer $A_i$ which would be converted into natural language response $R_i$. The dialogue acts of the utterances (e.g. INFORM\_SQL, CONFIRM\_SQL) are on the third column. Interaction turns are separated by the white area.}
\label{tab:CoSQL} % is used to refer this table in the text
 \vspace{-4mm}
\end{table}
